Fast Randomized Algorithms for t-Product Based Tensor Operations and Decompositions with Applications to Imaging Data

Tensors of order three or higher have found applications in diverse fields, including image and signal processing, data mining, biomedical engineering and link analysis, to name a few. In many applications that involve for example time series or other ordered data, the corresponding tensor has a distinguishing orientation that exhibits a low tubal structure. This has motivated the introduction of the tubal rank and the corresponding tubal singular value decomposition in the literature. In this work, we develop randomized algorithms for many common tensor operations, including tensor low-rank approximation and decomposition, together with tensor multiplication. The proposed tubal focused algorithms employ a small number of lateral and/or horizontal slices of the underlying 3-rd order tensor, that come with {\em relative error guarantees} for the quality of the obtained solutions. The performance of the proposed algorithms is illustrated on diverse imaging applications, including mass spectrometry data and image and video recovery from incomplete and noisy data. The results show both good computational speed-up vis-a-vis conventional completion algorithms and good accuracy.

==> Abstract_ver01.tex <==
	%\vspace{0.5cm}
\begin{abstract}
Tensors of order three or higher have found applications in diverse fields, including image and signal processing, data mining, biomedical engineering and link analysis, to name a few. In many applications that involve for example time series or other ordered data, the corresponding tensor has a distinguishing orientation that exhibits a low tubal structure.
This has motivated the introduction of the tubal rank and the corresponding tubal singular value decomposition in the literature. 
In this work, we develop randomized algorithms for many common tensor operations, including tensor low-rank approximation and decomposition, together with tensor multiplication. The proposed tubal focused algorithms employ a small number of lateral and/or horizontal slices of the underlying 3-rd order tensor, that come with {\em relative error guarantees} for the quality of the obtained solutions. The performance of the proposed algorithms is illustrated on diverse imaging applications, including mass spectrometry data and image and video recovery from incomplete and noisy data. The results show both good computational speed-up vis-a-vis conventional completion algorithms and good accuracy. 
\end{abstract}

\begin{keywords}
tensor slices selection, circulant algebra, low rank decomposition, nuclear norm minimization
\end{keywords}

\begin{AMS}
  15A69, 15A23, 68W20, 65F30
\end{AMS} 

==> Acknowledgments_ver01.tex <==
\section*{Acknowledgments}
The authors would like to thank the Associate Editor and three anonymous referees for many constructive comments and suggestions that improved significantly the structure and readability of the paper. 

==> Multiplication_ver01.tex <==
%
%In this section, we present a randomized tensor-product and provide the key results on the quality of the approximation.
%Given two tensors $\T{A}$ and $\T{B}$, using Definition~\ref{circ}, the t-product may be written as follows:
%\begin{equation}\label{prods}
%  \T{A}*\T{B} = \sum_{t=1}^{n_2}\T{A}_{:t:}*\T{B}_{t::},
%\end{equation}
%where $*$ denotes the tensor product.
%
%It can be easily shown that the left hand side of \eqref{prods} is equivalent to the block multiplication and then summation in the Fourier domain. When a tensor multiplication is formulated as \eqref{prods}, we can develop a randomized algorithm to approximate the product $\T{A}*\T{B}$.
%
%Algorithm~\ref{alg:matrix multiply} takes as input two tensors $\T{A}$ and $\T{B}$, positive integer $ c \le n_2$, and a probability distribution $\{p_i\}_{i=1}^{n_2}$ over $[n_2]$. It returns as output two tensors $\T{C}$ and $\T{R}$, where the lateral slices of $\T{C}$ are a small number of sampled and rescaled slices of $\T{A}$ and similarly the horizontal slices of $\T{R}$ constitute a small number of sampled and rescaled slices of $\T{B}$. Formally speaking, assume that at most $c$ lateral slices (in expectation) of $\T{A}$ are chosen by including the $i$-th lateral slice of $\T{A}$ in $\T{C}$ with probability $p_i = \min \{1,cp_i\}$. Then, define the sampling tensor $\T{S} \in \mathbb{R}^{n_2 \times n_2 \times n_3}$ to be the zero-one tensor where $S_{ii1} = 1$ if the $i$-th slice is chosen and $\T{S}_{ij2:n_3} = 0$ otherwise, and define the rescaling tensor $\T{D} \in \mathbb{R}^{n_2 \times c \times n_3}$ to be the tensor with $\T{D}_{ij1} = 1/\sqrt{cp_{j}}$ if $i-1$ of the previous slices have been chosen and $\T{D}_{ij2:n_3}=0$ otherwise. Similarly, the \texttt{rt-product} sample and rescale the corresponding horizontal slices of the tensor $\T{B}$. In both of these cases, $\T{C} = \T{A}* \T{S}*\T{D}$ is an $n_1 \times c \times n_3$ tensor consisting of sampled and rescaled copies of the lateral slices of $\T{A}$, and $\T{R} = (\T{S}*\T{D})^\top *\T{B} = \T{D}*\T{S}^\top *\T{B}$ is a $c \times n_2 \times n_3$ tensor consisting of sampled and rescaled copies of the horizontal slices of $\T{B}$. For the case of $n_3=1$, the algorithm chooses column-row pairs in Algorithm~\ref{alg:matrix multiply} and is identical to the algorithm of \cite{drineas2006fast}.
%
%\begin{algorithm}[h]
%\caption{\texttt{(rt-product)}, a fast Monte-Carlo algorithm for approximate tensor multiplication.}\label{alg:matrix multiply}
%\begin{algorithmic}[1]
%\STATE{ \textbf{Input}: $\T{A} \in \mathbb{R}^{n_1 \times n_2 \times n_3}$, $\T{B} \in \mathbb{R}^{n_2 \times n_4 \times n_3}$, $p_i \geq 0, i\in[n_2]$ s.t. $\sum_{i \in [n_2]}p_i=1$, positive integer $c \leq n_2$.}
%\STATE{Initialize $\T{S} \in \mathbb{R}^{n_2 \times n_2 \times n_3} $ and $\T{D} \in \mathbb{R}^{n_2 \times c \times n_3}$ to the all zeros tensors.}
%\STATE{$t=1$;}
%\FOR{$i=1, \dots, n_2$}%(construct sampling and rescaling tensors)\\
%\STATE{Pick $i$ with probability $\min\{1,c p_i\}$;}
%\IF{$i$ is picked}
%\STATE{$\T{S}_{it1} = 1, \quad \T{S}_{it2:n_3} =0$;}
%\STATE{$\T{D}_{tt1} = 1/\min\{1,\sqrt{cp_{i}}\}, \quad \T{D}_{tt2:n_3} =0;$}
%\STATE{$t = t + 1$\;}
%\ENDIF
%\ENDFOR
%\STATE{$\T{C} = \T{A}*\T{S}*\T{D}$,  \quad $\T{R} = \T{D}* \T{S}^\top * \T{B} $;}
%\STATE{$\hat{\T{C}} \leftarrow \texttt{fft}(\T{C}, [], 3)$, \quad  $\hat{\T{R}} \leftarrow \texttt{fft}(\T{R}, [], 3)$;}
%\FOR{$k=1, \dots, n_3$}
%\STATE{$ \hat{\T{Z}}_{::k}= \hat{\T{C}}_{::k}\hat{\T{R}}_{::k};$}
%\ENDFOR\\
%\STATE{$\T{Z} \leftarrow \texttt{ifft}(\hat{\T{Z}}, [], 3);$}\\
%\RETURN  $\T{Z}$
%\end{algorithmic}
%\end{algorithm}
%%-----------------------------------------------------------------------
% \subsection{Running time of rt-product}
%
% The \texttt{rt-product} is straightforward to implement, is computationally efficient, has small memory requirements,
%and is well suited for large scale problems. Indeed, the \texttt{rt-product} algorithm can be implemented without storing the tensors $\T{A} \in \mathbb{R}^{n_1 \times n_2 \times n_3}$ and $\T{B} \in \mathbb{R}^{n_2 \times n_4 \times n_3}$ and uses $O(\max (n_1,n_4) c n_3 \log(n_3))$ flops to transform to the Fourier domain and $O( c (n_1 +n_2 + n_4) n_3)$ flops to construct $\T{C}\in \mathbb{R}^{n_1\times c \times n_3}$ and $\T{R}\in \mathbb{R}^{c \times n_4 \times n_3}$, where \begin{equation}\label{multi:approx}
%\T{A}*\T{B}\sim \T{C}*\T{R}.
%\end{equation}
%It is worth mentioning that we do not require storing the sampling and rescaling tensors $\T{S}$ and $\T{D}$ in ourl implementation.
%\subsection{Approximate tensor multiplication: theoretical analysis}



==> Proof_of_Uniform_Theorem.tex <==
\subsection{Proof of Corollary~\lowercase{\ref{cor:proj-main}}: }
\label{sec:proj-proof}
%
Fix $c = 48000/\log(1/0.45)$, and notice that for $n > 1$,
$$48000\log(n) \geq 3200\log(n^5) \geq 3200\log(16n).$$
Hence $l \geq 3200r\mu_0(\T{V}_{L})\log(16n)(\log(\delta)/\log(0.45))/\epsilon^2.$

Now partition the columns of $\T{C}$ into $b = \log(\delta)/\log(0.45)$ 
submatrices, $\T{C}=[\T{C}_1,\cdots,\T{C}_b]$, each with $a=l/b$ columns,\footnote{For simplicity, 
we assume that $b$ divides $l$ evenly.}
and let $[\T{L}_{C_1},\cdots,\T{L}_{C_b}]$ be the corresponding partition of $\T{L}_C$.
Since 
$$a \geq 3200r\mu_0(\T{V}_{L})\log(4n/0.25)/\epsilon^2,$$
we may apply Prop.~\ref{prop:regress} independently for each $i$ to yield
\begin{equation}
\label{eqn:subblock-succ}
\norm{\T{M} - \T{C}_i\pinv{\T{L}_{C_i}}\T{L}}_F \leq (1+\epsilon)\norm{\T{M} - \T{M}\pinv{\T{L}}\T{L}}_F
\leq (1+\epsilon)\norm{\T{M} - \T{L}}_F
\end{equation}
with probability at least $0.55$, since $\T{M}\pinv{\T{L}}$ minimizes
$\norm{\T{M}-\T{Y}\T{L}}_F$ over all $\T{Y}\in\mathbb{R}^{m\times m}$.

Since each $\T{C}_i = \T{C}\T{S}_i$ for some matrix $\T{S}_i$ and $\pinv{\T{C}}\T{M}$ minimizes $\norm{\T{M}-\T{C}\T{X}_F$ over all
$\T{X}\in\mathbb{R}^{l\times n}$, it follows that
$$\norm{\T{M}-\T{C}{\T{C}}^\dagger \T{M}}_F\leq\norm{\T{M}-\T{C}_i\pinv{\T{L}_{C_i}}\T{L}}_F,$$
for each $i$.
Hence, if 
$$\norm{\T{M} - \T{C}\T{C}^+\T{M}}_F \leq (1+\epsilon)\norm{\T{M} - \T{L}}_F,$$
fails to hold, then, for each $i$, \eqref{eqn:subblock-succ} also fails to hold.
The desired conclusion therefore must hold with probability at least
$1-0.45^b = 1-\delta$.

==> Proofofsliceprojmain_ver01_copy.tex <==
\subsection{Proof of Corollary~\ref{cor:proj-main}}
\label{cor:proj-main-proof}

Since $\T{C}^+*\T{A}$ minimizes $\|\T{A}-\T{C}*\T{X}\|_F$ over all tensors $\T{X} \in \mathbb{R}^{n_1 \times c \times n_3}$, it follows that $$\|\T{A}-\T{C}*\T{C}^\dagger*\T{A}\|_F\leq\|\T{A}-\T{C}*\T{L}_{\T{C}}^\dagger*\T{L}\|_F.$$

Now, using  \eqref{eq:prop:regress}, we get 
\begin{equation}\label{eq:tcx:constant}
 \|\T{A} - \T{C}*\T{C}^\dagger*\T{A}\|_F \leq (1+\epsilon)\|\T{A} - \T{L}\|_F,
\end{equation} 
 with probability at least $0.85$.

%Similar to the proof of Theorem~\ref{thm:regress-main}, we can use Proposition \ref{prop:regress} with probability at least 0.85 and then apply an analogous boosting method.  
%
We can trivially boost the success probability to $1-\delta$ by repeating Algorithm~\ref{alg:algCX} $O (\log (1/\delta))$ rounds. Specifically, let $\T{C}_i$ denote the output of Algorithm~\ref{alg:algCX} at round $i$;  using \eqref{eq:tcx:constant} for each $\T{C}_i $ we have
\begin{equation}
\label{eqn:rela}
\|\T{A}  - \T{C}_i * \T{C}_i^\dagger*\T{A}\|_F\leq (1+\epsilon)\|\T{A} - \T{L}\|_F,  
\end{equation}
with probability at least $0.85$.

Now, let $\T{C}$ denote the set of all columns used in the approximation. Since  each $\T{C}_i = \T{C} * \T{S}_i$ for some tensor $\T{S}_i$ and $\T{C}^+*\T{A}$ minimizes $\|\T{A}-\T{C}*\T{X}\|_F$ over all tensors $\T{X} \in \mathbb{R}^{n_1 \times c \times n_3}$, it follows that $$\|\T{A}-\T{C}*\T{C}^\dagger*\T{A}\|_F\leq\|\T{A}-\T{C}_i*\T{C}_i^\dagger*\T{A}\|_F,$$ 
for each $i$.  
Hence, if 
$$ \|\T{A} - \T{C}*\T{C}^\dagger*\T{A}\|_F \leq (1+\epsilon)\|\T{A} - \T{L}\|_F,$$
fails to hold, then for each $i$, \eqref{eqn:rela} also fails to hold.
Since $0.15< 1/e$, the desired conclusion must hold with probability at least $1- (1/e)^{\log (1/\delta)}  = 1-\delta$.
%
% 
% 
%The inequality \eqref{eq:tcx:constant} holds with probability at least $1-\delta$ by following the boosting strategy employed in the proof of Theorem~\ref{thm:regress-main}. 

  

==> proofofcorollarymultipication_ver01.tex <==
\subsection{Proof of Corollary~\ref{lem:mat-mult}}
\label{lem:mat-mult-proof}


Once Theorem~\ref{theorem:matmult-main-exact} is substituted for Theorem~7 of \cite{drineas2008relative}, the proof of this corollary follows similarly from \cite{hsu2012tail}.


==> proofofmaint-CUR.tex <==
\section{Proof of Corollary~\lowercase{\ref{cor:gnys-main}}:}
\label{sec:gnys-proof}
%

Using Theorem.~\ref{thm:regress-main} and Proposition~\ref{cor:proj-main} it follows that
$$\|\T{A} - \T{C}*\T{U}*\T{R}\|_F \leq (1+\epsilon)\|\T{A} - \T{C}^+*\T{C}*\T{A}\|_F
\leq (1+\epsilon)^2\norm{\T{A} - \T{L}}$$
with probability at least $(1-\delta)(1-\delta' - 0.2)$ by independence.


==> proofofmainuniformt-CX.tex <==
\subsection{Proof of Corollary~\lowercase{\ref{cor:proj-main}}: }
\label{sec:proj-proof}
%
Fix $c = 48000/\log(1/0.45)$, and notice that for $n > 1$,
$$48000\log(n) \geq 3200\log(n^5) \geq 3200\log(16n).$$
Hence $l \geq 3200r\mu_0(\T{V}_{L})\log(16n)(\log(\delta)/\log(0.45))/\epsilon^2.$

Now partition the columns of $\T{C}$ into $b = \log(\delta)/\log(0.45)$ 
submatrices, $\T{C}=[\T{C}_1,\cdots,\T{C}_b]$, each with $a=l/b$ columns,\footnote{For simplicity, 
we assume that $b$ divides $l$ evenly.}
and let $[\T{L}_{C_1},\cdots,\T{L}_{C_b}]$ be the corresponding partition of $\T{L}_C$.
Since 
$$a \geq 3200r\mu_0(\T{V}_{L})\log(4n/0.25)/\epsilon^2,$$
we may apply Prop.~\ref{prop:regress} independently for each $i$ to yield
\begin{equation}
\label{eqn:subblock-succ}
\norm{\T{M} - \T{C}_i\pinv{\T{L}_{C_i}}\T{L}}_F \leq (1+\epsilon)\norm{\T{M} - \T{M}\pinv{\T{L}}\T{L}}_F
\leq (1+\epsilon)\norm{\T{M} - \T{L}}_F
\end{equation}
with probability at least $0.55$, since $\T{M}\pinv{\T{L}}$ minimizes
$\norm{\T{M}-\T{Y}\T{L}}_F$ over all $\T{Y}\in\mathbb{R}^{m\times m}$.

Since each $\T{C}_i = \T{C}\T{S}_i$ for some matrix $\T{S}_i$ and $\pinv{\T{C}}\T{M}$ minimizes $\norm{\T{M}-\T{C}\T{X}_F$ over all
$\T{X}\in\mathbb{R}^{l\times n}$, it follows that
$$\norm{\T{M}-\T{C}{\T{C}}^\dagger \T{M}}_F\leq\norm{\T{M}-\T{C}_i\pinv{\T{L}_{C_i}}\T{L}}_F,$$
for each $i$.
Hence, if 
$$\norm{\T{M} - \T{C}\T{C}^+\T{M}}_F \leq (1+\epsilon)\norm{\T{M} - \T{L}}_F,$$
fails to hold, then, for each $i$, \eqref{eqn:subblock-succ} also fails to hold.
The desired conclusion therefore must hold with probability at least
$1-0.45^b = 1-\delta$.

==> shared_ver02.tex <==
% SIAM Shared Information Template
% This is information that is shared between the main document and any
% supplement. If no supplement is required, then this information can
% be included directly in the main document.


% Packages and macros go here
\usepackage{lipsum}
\usepackage{amsfonts}
\usepackage{graphicx}
\usepackage{epstopdf}
\usepackage{algorithmic}
\usepackage{mathrsfs, amsmath, amscd, amssymb}
\usepackage[mathscr]{euscript} %% Tensor
\usepackage{subcaption} %% Subfigure
%%%%%%%%%%%
%\usepackage{mathptmx}      % use Times fonts if available on your \usepackage{latexsym}
%\usepackage{multirow}
%\usepackage{epsfig}
%\usepackage{verbatim}
%\usepackage{booktabs}
%\usepackage{graphicx}
%\usepackage{graphicx}
%\usepackage{stackrel}
%\usepackage{fancyhdr}
%\usepackage{makeidx}
%\usepackage{afterpage}
%\usepackage{hyperref}
%\usepackage{url}
%\usepackage{varwidth}
%\usepackage{bbm}
%\usepackage{hyperref}
%\usepackage{caption}
%\usepackage{subcaption}
%\usepackage{enumerate}
%\usepackage{theorem}
%\usepackage{amsthm}
%\usepackage{longtable}
%\usepackage{lscape}
%\usepackage[bookmarksnumbered, colorlinks, plainpages]{hyperref}
%\usepackage{colortbl}
%\usepackage{xcolor}
%\usepackage{array,booktabs}
%\usepackage{algorithm,algpseudocode}
%%%%%%%%%%
%\ifpdf
%  \DeclareGraphicsExtensions{.eps,.pdf,.png,.jpg}
%\else
%  \DeclareGraphicsExtensions{.eps}
%\fi

%strongly recommended
\numberwithin{theorem}{section}

% Declare title and authors, without \thanks
%\newcommand{\TheTitle}{FAST MONTE CARLO ALGORITHMS FOR TENSOR OPERATIONS}
%\newcommand{\TheAuthors}{D. Ataee Tarzanagh, and G. Michailidis}

% Sets running headers as well as PDF title and authors
%\headers{\TheTitle}{\TheAuthors}

% Title. If the supplement option is on, then "Supplementary Material"
% is automatically inserted before the title.
\title{{\TheTitle}\thanks{Submitted. \funding{This work was supported in part by NSF grants DMS-1545277, DMS-1632730, NIH grant1R01-GM1140201A1 and by the UF Informatics Institute.}}}

% Authors: full names plus addresses.
\author{
Davoud Ataee Tarzanagh\thanks{Department of Mathematics \& UF Informatics Institute, University of Florida, Gainesville, FL, \email{tarzanagh@ufl.edu}.}
  \and
George Michailidis\thanks{Department of Statistics \& UF Informatics Institute, University of Florida, Gainesville, FL, \email{gmichail@ufl.edu}.}
}
\usepackage{amsopn}


%tensor tube
\newcommand{\tube}[1]{\boldsymbol{\dot{\mathfrak{\MakeLowercase{#1}}}}}
%tensor column
\newcommand{\tcol}[1]{\boldsymbol{\mathring{\mathfrak{\MakeLowercase{#1}}}}}
%tensor vectorized
\newcommand{\tvec}[1]{\boldsymbol{\vec{\mathfrak{\MakeLowercase{#1}}}}}

%% Tensor notation
\newcommand{\T}[1]{\boldsymbol{\mathscr{\MakeUppercase{#1}}}} %tensor
\newcommand{\TLS}[2]{\M{#1}_{[#2]}} % lateral slice
\newcommand{\TFS}[2]{\M{#1}_{#2}} % frontal slice
\newcommand{\TT}[2]{\V{#1}_{#2}} % tube
\newcommand{\TE}[2]{\MakeLowercase{#1}_{#2}} % tensor element

%% Matrix & Tensor Operations
\newcommand{\Circ}[1]{{\rm circ}\left( #1 \right)}
\newcommand{\Fold}[1]{{\rm fold}\left( #1 \right)}
\newcommand{\Unfold}[1]{{\rm unfold}\left( #1 \right)}
\newcommand{\Twist}[1]{{\rm twist}(\M{#1})}
\newcommand{\Squeeze}[1]{{\rm squeeze}(#1)}
\newcommand{\squeeze}{{\rm squeeze}}
\newcommand{\Mout}{\diamondsuit}
\newcommand{\circu}{ {\rm circ}}
\newcommand{\bcirc}{ {\rm bcirc}}
\newcommand{\vvec}{ {\rm vec}}
%% Expectation
\newcommand{\Ec}{ \mathbf{E}}

\DeclareMathOperator{\Grad}{Grad}
\DeclareMathOperator{\codim}{codim}
\DeclareMathOperator{\ind}{ind}
\DeclareMathOperator{\Span}{span}
\DeclareMathOperator{\var}{var}
\DeclareMathOperator{\spec}{spec}
\DeclareMathOperator{\Aut}{Aut}
\DeclareMathOperator{\lin}{lin}
\DeclareMathOperator{\rank}{rank}


\DeclareMathOperator*{\argmin}{argmin}
\DeclareMathOperator*{\minimize}{minimize}
\DeclareMathOperator{\trace}{trace}
\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\diag}{diag}


%%% Local Variables:
%%% mode:latex
%%% TeX-master: "ex_article"
%%% End:

